Parallel Optimization of Polynomials for Large-scale Problems in Stability and Control

In this thesis, we focus on some of the NP-hard problems in control theory. Thanks to the converse Lyapunov theory, these problems can often be modeled as optimization over polynomials. To avoid the problem of intractability, we establish a trade off between accuracy and complexity. We develop a sequence of tractable optimization problems - in the form of LPs and SDPs - whose solutions converge to the exact solution of the NP-hard problem. However, the computational and memory complexity of these LPs and SDPs grow exponentially with the progress of the sequence - meaning that improving the accuracy of the solutions requires solving SDPs with tens of thousands of decision variables and constraints. Setting up and solving such problems is a significant challenge. The existing optimization algorithms and software are only designed to use desktop computers or small cluster computers - machines which do not have sufficient memory for solving such large SDPs. This in fact is the reason we seek parallel algorithms for setting-up and solving large SDPs on supercomputers. We propose parallel algorithms for stability analysis of two classes of systems: 1) Linear systems with a large number of uncertain parameters; 2) Nonlinear systems defined by polynomial vector fields. First, we develop a distributed parallel algorithm which applies Polya's and Handelman's theorems to some variants of parameter-dependent Lyapunov inequalities with parameters defined over the simplex. The result is a sequence of SDPs which possess a block-diagonal structure. We then develop a parallel SDP solver which exploits this structure to map the computation, memory and communication to a distributed parallel environment. Numerical tests on a supercomputer demonstrate the ability of the algorithm to efficiently utilize hundreds and potentially thousands of processors and analyze systems with 100+ dimensional state-space.

==> abstract.tex <==

\begin{abstract}
One of the greatest challenges in the field of mathematical programming is solving large-scale optimization problems. These problems are of growing interest to the engineering community as well, mainly because nowadays there are numerous real-world decision-making problems which can be modelled as large-scale optimization problems. Problems such as Economic Dispatch in power systems, Frequency Assignment in large mobile communication networks, and optimal control and operation of smart-grids can all be closely modelled as large-scale combinatorial/continuous optimization problems. Despite impressive advances in the development of optimization algorithms and commercial off-the-shelf optimization software, realistic optimization problems often fall into the class NP-hard.

We focus on some of the NP-hard problems in control theory which can be modelled as optimization over polynomials. To solve the problem of inherent intractability, we establish a trade off between accuracy and complexity. We develop a sequence of polynomial-time optimization problems - in the form of Linear Programs and/or Semi-Definite Programs - whose solutions converge to the exact solution of the NP-hard problem. Although there exist excellent algorithms and commercial software for solving LPs and SDPs efficiently, the computational and memory complexity of these LPs and SDPs grow exponentially with the progress of the sequence (accuracy). Hence, the complexity of these SDPs can rapidly grow beyond the memory and computational capacity of desktop and/or small cluster computers. This in fact, is the reason we seek parallel algorithms for setting-up the sequence of SDPs and solving them using large cluster computers.

In particular, we propose parallel computation for robust stability analysis of linear systems with parametric uncertainty and nonlinear systems defined by polynomial vector fields. First, we develop distributed parallel algorithms which apply Polya's and Handelman's theorems to some variants of parameter-dependent Lyapunov inequalities with parameters defined over the simplex, hypercubes and/or arbitrary convex polytopes. The results is a sequence of block-diagonal-structured SDPs. We then develop a parallel SDP solver which exploits this structure to map the computation, memory and communication to a distributed parallel environment. We produce Message Passing Interface implementations of our algorithms and provide theoretical and experimental analysis on complexity and scalability.
\end{abstract}

==> ack.tex <==
{Enter your acknowledgement text here}
